Fewer Tokens and Fewer Videos: Extending Video Understanding Abilities in Large Vision-Language Models

Amidst the advancements in image-based Large Vision-Language Models (image-LVLM), the transition to video-based models (video-LVLM) is hindered by the limited availability of quality video data. This paper addresses the challenge by leveraging the visual commonalities between images and videos to efficiently evolve image-LVLMs into video-LVLMs. We present a cost-effective video-LVLM that enhances model architecture, introduces innovative training strategies, and identifies the most effective types of video instruction data. Our innovative weighted token sampler significantly compresses the visual token numbers of each video frame, effectively cutting computational expenses. We also find that judiciously using just 10% of the video data, compared to prior video-LVLMs, yields impressive results during various training phases. Moreover, we delve into the influence of video instruction data in limited-resource settings, highlighting the significance of incorporating video training data that emphasizes temporal understanding to enhance model performance. The resulting Fewer Tokens and Fewer Videos LVLM (FTFV-LVLM) exhibits exceptional performance across video and image benchmarks, validating our model's design and training approaches.

==> sec/imagebenchmark.tex <==
% method~\cite{} & InternLM-7B & 224 & ehub & mmb & mmb^cn & seed^I \\ 






% method~\cite{} & InternLM-7B & 224 & vqav2 & gqa & vizwiz & sqa & tvqa & pope & mme & mmb & mmbcn & seed & llavaw & mmvet \\ 

% \begin{table*}[ht]
% \center
% \begin{small}
% \resizebox{1.0\textwidth}{!}
% {
% \begin{tabular}{ccc|ccccc|ccccccc}
% \toprule
% \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{LLM}} & \multirow{2}{*}{\textbf{Res.}} & \multicolumn{5}{c|}{\textbf{Image Question Answering}} & \multicolumn{7}{c}{\textbf{Image Benchmark Toolkit}} \\
%  & & & VQA$^{\text{v2}}$& GQA& VisWiz& SQA$^\text{I}$& VQA$^{\text{T}}$&  POPE& MME& MMB& MMB$^{\text{CN}}$& SEED$^\text{I}$& LLaVA$^{\text{W}}$& MM-Vet \\
%  \midrule
% mPLUG-Owl~\cite{ye2023mplug} & LLaMA-7B & 224 & - & 14.0 & 39.0 & 2.8 & 38.8 & - & - & 46.6 & - & - & - & - \\ 
% Otter~\cite{li2023otter} & LLaMA-7B & 224 & - & 38.1 & 50.0 & 27.2 & 21.2 & - & - & 32.6 & - & - & - & 24.6 \\ 
% IDEFICS-9B~\cite{idefics} &  LLaMA-7B & 224 & 50.9 & 38.4 & 35.5 & - & 25.9 & - & - & 48.2 & 25.2 & - & - & - \\ 
% InstructBLIP~\cite{instructblip} & Vicuna-7B & 224 & - & 49.2 & 34.5 & 60.5  & 50.1 & - & - & 36 &  23.7 & 58.8 &  60.9 & 26.2 \\
% Qwen-VL~\cite{bai2023qwen} & Qwen-7B & 448 & 79.5 & 59.3 & 35.2 & 67.1 & 63.8 & - & - & 38.2 & 7.4 & 62.3 & - & - \\
% Qwen-VL-Chat~\cite{bai2023qwen} & Qwen-7B & 448 & 78.2 & 57.5 & 38.9 & 68.2 & 61.5 & - & 1487.5 & 60.6 & 56.7 & 65.4 & - & - \\
% MiniGPT-v2~\cite{chen2023minigpt} & LLaMA2 7B &448 & - & 60.3 & 32.9 & - & - & - & - & - & - & - & - & - \\ 
% MiniGPT-v2-Chat~\cite{chen2023minigpt} & LLaMA2-Chat 7B & 448 & - & 60.1 & 53.6 & - & - & - & - & - & - & - & - & - \\ 
% LLaVA-1.5~\cite{liu2023improved}& Vicuna-7B& 336&  78.5& 62.0& 50.0& 66.8& 58.2& 85.9& 1510.7& 64.3& 58.3& -& 63.4&  30.5 \\
% InternLM-XComposer-VL~\cite{zhang2023internlm} & InternLM-7B & 224 & - & - & - & - & - & - & 1528.4 & 74.8 & 73.1 & 66.9 & - & - \\ 
% % LLaVA-1.5~\cite{liu2023improved}& Vicuna-13B&  336& 80.0& 63.3& 53.6& 71.6& 61.3& 85.9& 1531.3& 67.7& 63.6&  61.6&  70.7& 35.4 \\
% Video-LLaVA~\cite{lin2023video} & Vicuna-7B & 224 & 74.7 & 60.3 & 48.1 & 66.4  & 51.8 & 84.4 & - & 60.9 & - & - & 73.1 & 32.0 \\
% LLaMA-VID~\cite{li2023llama} & Vicuna-7B & 336 & 79.3 & 64.3 & 54.2 & 68.3 & - & 86.0 & 1521.4 & 65.1 & - & 67.6 & - & - \\ 
% \bottomrule
% \end{tabular}
% }
% \end{small}
% \caption{Comparison with SoTA methods on 12 image understanding benchmarks. Res indicates input image resolution. Benchmark names are abbreviated due to space limits. VQA$^{\text{v2}}$~\cite{goyal2017making}; GQA~\cite{hudson2019gqa}; VisWiz~\cite{gurari2018vizwiz}; SQA$^\text{I}$: ScienceQA-IMG~\cite{lu2022learn};
% VQA$^{\text{T}}$: TextVQA~\cite{singh2019towards}; POPE~\cite{li2023evaluating}; MME~(perception)~\cite{fu2023mme}; MMB: MMBench~(dev)~\cite{liu2023mmbench}; MMB$^{\text{CN}}$: MMBench-Chinese~(dev)~\cite{liu2023mmbench}; SEED$^\text{I}$: SEED-Bench~(image)~\cite{li2023seed};
% LLaVA$^{\text{W}}$: LLaVA-Bench~(In-the-Wild)~\cite{liu2023visual}; MM-Vet~\cite{yu2023mm}.}\label{tab:image_benchmark}
% \end{table*}




==> sec/videobenchmark.tex <==

\begin{table*}[ht]
\center
\begin{small}
\resizebox{1.0\textwidth}{!}
{
\begin{tabular}{ccc|cccccc|ccccc}
\toprule
\multirow{2}{*}{\textbf{Method}} & 
\multirow{2}{*}{\textbf{LLM}} & 
\multirow{2}{*}{\textbf{Res.}} &
\multicolumn{2}{c}{\textbf{MSVD-QA}} & 
\multicolumn{2}{c}{\textbf{MSRVTT-QA}} & 
\multicolumn{2}{c|}{\textbf{ActivityNet-QA}} & 
\multicolumn{5}{c}{\textbf{Video-based Generative Performance Benchmarking}} \\
& & & Acc & Score & Acc & Score & Acc & Score & Correctness & Detail & Context & Temporal &  Consistency\\
\midrule
FrozenBiLM~\cite{yang2022zero} & DeBERTa-V2 & 224 & 32.2 & - & 16.8 & - & 24.7 & - & - & - & - & - & - \\
VideoLLaMA~\cite{zhang2023video} & Vicuna-7B & 224 & 51.6 & 2.5 & 29.6 & 1.8 & 12.4 & 1.1 & 1.96 & 2.18 & 2.16 & 1.82 & 1.79\\
LLaMA-Adapter~\cite{zhang2023llama} & LLaMA-7B & 224 & 54.9 & 3.1 &  43.8 & 2.7 & 34.2 & 2.7 & 2.03 & 2.32 & 2.30 & 1.98 & 2.15 \\
VideoChat~\cite{li2023videochat} & Vicuna-7B & 224 & 56.3 & 2.8 & 45.0 & 2.5 & 26.5 & 2.2 & 2.23 & 2.50 & 2.53 & 1.94 & 2.24\\
Video-ChatGPT~\cite{maaz2023video} & Vicuna-7B & 224 & 64.9 & 3.3 & 49.3 &  2.8 & 35.2 & 2.7 & 2.40 & 2.52 & 2.62 & 1.98 & 2.37\\
Valley$^{*}$~\cite{luo2023valley} & Vicuna-7B & 224 & xxx & xxx & xxx & xxx & xxx & xxx & xxx & xxx & xxx & xxx & xxx\\
BT-Adapter~\cite{liu2023one} & Vicuna-7B & - & 67.5 & 3.7 & 57.0 & 3.2 & 45.7 & 3.2 & 2.68 & 2.69 & 3.27 & 2.34 & 2.46 \\
VideoChat2 & Vicuna-7B & 224&70.0&3.9&54.1&3.3&49.1&3.3 &3.02&2.88&3.51&2.66&2.81 \\
Video-LLaVA~\cite{lin2023video} & Vicuna-7B & 224 & 70.7 & 3.9 & 59.2 & 3.5 & 45.3 &  3.3 & - & - & - & - & -\\
LLaMA-VID~\cite{li2023llama} & Vicuna-7B & 224 & 69.7 & 3.7 & 57.7 & 3.2 & 47.4 & 3.3 & 2.96 & 3.00 & 3.53 & 2.46 & 2.51\\
\midrule
FTFV-LLM_{S4-V} (ours) & Vicuna-7B & 448 & 69.18 & 3.73 & 55.06 & 3.14 & 49.67 & 3.31 & 2.61 &2.74  & 3.13 & 2.20 &2.29 \\
FTFV-LLM_{S3-IV} (ours) & Vicuna-7B & 448 & 70.25 &  3.77& 53.36 & 3.13 &52.22  &3.39  & 2.69 & 2.83 & 3.27 & 2.30 & 2.50\\
FTFV-LLM_{S2-S3-IV} (ours) & Vicuna-7B & 448 & 68.89 & 3.74 & 51.97 & 3.08 & 52.00 & 3.36 &2.73 &2.83 &3.30  &2.32 & 2.46\\

\bottomrule
\end{tabular}
}
\end{small}
\caption{Comparison with leading methods on Video-QA benchmark and  Video-based Generative Performance benchmark~\cite{maaz2023video}. Res indicates input image and video frame resolution. *: We get Valley~(Vicuna-7B) results by testing their provided model checkpoint in the video benchmarks. }
\label{tab:video_benchmark_chatgpt}
\end{table*}




\begin{table}
\center
\resizebox{1.0\columnwidth}{!}
{
\begin{tabular}{c|cccc|c}
\toprule
\multirow{2}{*}{\textbf{Method}} & 
\multicolumn{4}{c|}{\textbf{VideoBench}} & 
\textbf{MVBench}  \\
& Exc & Prior & Dec & All & Avg \\
\midrule
VideoChat~\cite{li2023videochat}  & 34.12 & 29.61 & 42.50 & 35.41 & 35.5 \\
Video-ChatGPT~\cite{maaz2023video} & 39.82 & 29.24 & 46.50 & 38.52 & 32.7 \\
Otter~\cite{li2023otter}  & 37.52 & 32.99 & 41.90 & 37.47 & 26.8 \\
PandaGPT~\cite{su2023pandagpt}  & 37.54 & 31.99 & 43.05 & 37.52 & - \\
Valley~\cite{luo2023valley}  & 28.39 & 29.21 & 44.27 & 33.96 & - \\
mPLUG-Owl~\cite{ye2023mplug}  & 33.17 & 26.40 & 39.88 & 33.15 & 29.7 \\
VideoLLaMA~\cite{zhang2023video}  & 32.48 & 27.80 & 38.21 & 32.83 & 34.1 \\
VideoChat2~\cite{li2023mvbench} & - & - & - & - & 51.1 \\ 
\midrule
FTFV-LLM_{S4-V} (ours)  & 54.31 & 42.01 & 54.45 &50.26& 43.52 \\
FTFV-LLM_{S3-IV} (ours)  &  &  &  &  &44.75 \\
FTFV-LLM_{S2-S3-IV} (ours)  &  &  &  &  & 44.15 \\


\bottomrule
\end{tabular}
}
\caption{Comparison of leading methods on the VideoBench~\cite{ning2023video} and MVBench~\cite{li2023mvbench} benchmarks. Subset names in VideoBench are abbreviated due to page limitations. Exc: Video-Exclusive Understand; Prior: Prior Knowledge-based Question-Answering; Dec: Comprehension and Decision-Making. }
\label{tab:video_bench}
\end{table}


\begin{table*}
\center
\begin{small}
\resizebox{0.9\textwidth}{!}
{
\begin{tabular}{c|cccccc|ccccc|c|c}
\toprule
\multirow{2}{*}{\textbf{Method}} & 
\multicolumn{2}{c}{\textbf{MSVD-QA}} & 
\multicolumn{2}{c}{\textbf{MSRVTT-QA}} & 
\multicolumn{2}{c|}{\textbf{ActivityNet-QA}} & 
\multicolumn{5}{c|}{\textbf{Video-based Generative Performance Benchmarking}} &
\multicolumn{1}{c|}{\textbf{Video-Bench}} & 
\textbf{MVBench} \\
& Acc & Score & Acc & Score & Acc & Score & Correctness & Detail & Context & Temporal &  Consistency& Avg&Avg\\
\midrule

S4-V_{10\%}  & 69.18 & 3.73 & 55.06 & 3.14 & 49.67 & 3.31 & 2.61 &2.74  & 3.13 & 2.20 &2.29 &50.26 &43.52\\
S4-V_{30\%} & 68.68 &  3.71& 55.13 & 3.16 &48.64  &3.31  & 2.69 & 2.78 & 3.18 & 2.22 & 2.26 & 50.12&44.0\\
S4-V_{60\%}  & 68.96 & 3.72 & 55.21 & 3.17 & 48.97 & 3.29 &2.71 &2.79 &3.22  &2.29 & 2.31 
& 50.36&43.73\\
S4-V_{100\%}  & 68.57 & 3.70 & 55.20 & 3.17 & 48.85 & 3.31 &2.78 &2.83 &3.23  &2.29 & 2.38 & 50.86&44.47\\
\midrule
S3-IV_{10\%}  & 70.25 & 3.77 & 53.36 & 3.13 & 52.22 & 3.39 & 2.69 &2.83  & 3.27 & 2.30 &2.49 & &44.75\\
S3-IV_{30\%} & 70.39 &  3.78& 55.25 & 3.18 &52.84  &3.41  & 2.64 & 2.80 & 3.20 & 2.35 & 2.49 &48.65 &44.28\\
S3-IV_{60\%}  & 69.23 & 3.77 & 54.53 & 3.15 & 52.08 & 3.39 &      &2.80 &3.25  &2.31 & 2.47 
& 49.89 &44.47\\
S3-IV_{100\%} & 69.55 & 3.78 & 54.50 & 3.17 & 51.54 & 3.40 &2.79 &2.84 &3.29  &2.33 & 2.40 & 48.62&44.3 \\
\midrule
S2-S3-IV_{10\%-10\%}  & 68.89 & 3.74 & 51.97 & 3.08 & 51.00 & 3.36 & 2.73 &2.83  & 3.30 & 2.32 &2.46 &50.12 &44.15\\
S2-S3-IV_{10\%-30\%}  & 69.51 & 3.75 & 53.77 & 3.15 & 51.75 & 3.41 & 2.76 &2.87  & 3.34 & 2.24 &2.55 &49.90 &44.75\\
S2-S3-IV_{10\%-60\%}  & 68.55 & 3.77 & 52.45 & 3.12 & 51.50 & 3.40 & 2.77 &2.85  & 3.32 & 2.28 &2.53 &49.75 &45.78\\
S2-S3-IV_{10\%-100\%} & 69.07 &  3.77& 52.96 & 3.15 &52.45  &3.39  & 2.85 & 2.88 & 3.33 & 2.34 & 2.55 &49.70 &44.80\\
S2-S3-IV_{100\%-100\%}  & 69.26 & 3.77 & 54.06 & 3.17 & 52.52 & 3.40 &2.79 &2.85 &3.31  &2.29 & 2.57 &49.97 &44.95\\
\bottomrule
\end{tabular}
}
\end{small}

\caption{Comparison with varying proportions of video training data on Video-QA benchmark and  Video-based Generative Performance benchmark~\cite{maaz2023video}. Res indicates input image and video frame resolution.  }
\label{tab:impact_of_videodata_amount}
\end{table*}


\begin{table*}
\center
\begin{small}
\resizebox{0.9\textwidth}{!}
{
\begin{tabular}{c|cccccc|cccccc|c|c|c}
\toprule
\multirow{2}{*}{\textbf{Method}} & 
\multicolumn{2}{c}{\textbf{MSVD-QA}} & 
\multicolumn{2}{c}{\textbf{MSRVTT-QA}} & 
\multicolumn{2}{c|}{\textbf{ActivityNet-QA}} & 
\multicolumn{6}{c|}{\textbf{Video-based Generative Performance Benchmarking}} &
\multicolumn{1}{c|}{\textbf{Video-Bench}} & 
\textbf{MVBench} &
\multirow{2}{*}{\textbf{Avg}} \\
& Acc & Score & Acc & Score & Acc & Score & Correctness & Detail & Context & Temporal &  Consistency& Avg&Avg&Avg \\
\midrule

S3-IV_{16}  & 68.61 & 3.78 &  &  & 50.82 & 3.32 & 2.66 &2.80  & 3.23 & 2.23 &2.47 &2.68& &44.70 &\\
S3-IV_{32} & 68.54 &  3.77& 47.09 & 2.92 &49.56  &3.29  & 2.67 & 2.76 & 3.23 & 2.28 & 2.53 & 2.69&48.37&44.80&43.51\\
S3-IV_{64}  & 69.15 & 3.79 & 51.94 & 3.10 & 50.71 & 3.36 &2.68 &2.82 &3.27  &2.29 & 2.50 &2.71&48.92&44.02&44.58\\
S3-IV_{128}  & 70.39 & 3.78 & 55.25 & 3.18 & 52.84 & 3.41 & 2.64 &2.80  & 3.20 & 2.35 &2.49 & 2.70&48.65&44.28&45.69\\
S3-IV_{256} & 70.29 &  3.79& 52.20 & 3.08 &50.91  &3.36  & 2.77 & 2.82 & 3.24 & 2.36 & 2.49&2.74& &44.73 &\\

\bottomrule
\end{tabular}
}
\end{small}

\caption{Comparison with different number of sample tokens on Video-QA benchmark and  Video-based Generative Performance benchmark~\cite{maaz2023video}. Res indicates input image and video frame resolution. }
\label{tab:impact_of_weighted_token_sampler}
\end{table*}


\begin{table*}
\center
\begin{small}
\resizebox{0.9\textwidth}{!}
{
\begin{tabular}{c|cccccc|ccccc|c|c}
\toprule
\multirow{2}{*}{\textbf{Method}} & 
\multicolumn{2}{c}{\textbf{MSVD-QA}} & 
\multicolumn{2}{c}{\textbf{MSRVTT-QA}} & 
\multicolumn{2}{c|}{\textbf{ActivityNet-QA}} & 
\multicolumn{5}{c|}{\textbf{Video-based Generative Performance Benchmarking}} &
\multicolumn{1}{c|}{\textbf{Video-Bench}} & 
\textbf{MVBench} \\
& Acc & Score & Acc & Score & Acc & Score & Correctness & Detail & Context & Temporal &  Consistency& Avg&Avg\\
\midrule

S3-IV_{randn}  & 69.18 & 3.73 & 55.06 & 3.14 & 49.67 & 3.31 & 2.61 &2.74  & 3.13 & 2.20 &2.29 & &\\
S3-IV_{weighted} & 70.25 &  3.77& 53.36 & 3.13 &52.22  &3.39  & 2.69 & 2.83 & 3.27 & 2.30 & 2.50 & &\\
\bottomrule
\end{tabular}
}
\end{small}
\caption{Comparison with different method to sample tokens on Video-QA benchmark and  Video-based Generative Performance benchmark~\cite{maaz2023video}. ‘Avg’ denotes the average results for each benchmark. For MSVD-QA, MSRVTT-QA, and ActivityNet-QA benchmarks, only their Acc scores were included in the average calculation. As for ~\cite{maaz2023video}, its average results were used to calculate the final Avg score. }
\label{tab:impact_of_weighted_token_sampler_method}
\end{table*}



\begin{table}
\center
\begin{small}
\resizebox{0.9\textwidth}{!}
{
\begin{tabular}{c|c}
\toprule
\multirow{2}{*}{\textbf{Method}} & 
\multicolumn{1}{c}{\textbf{MVBench}}  \\

\midrule
S4-V_{10\%_basic}  & \\
S4-V_{10\%_divercity} &\\
S3-IV_{10\%_basic}  & \\
S3-IV_{10\%_divercity} &\\
S3-IV_{30\%_basic}  & \\
S3-IV_{30\%_divercity} &\\

\bottomrule
\end{tabular}
}
\end{small}
\caption{Comparison with different method to sample tokens on Video-QA benchmark and  Video-based Generative Performance benchmark~\cite{maaz2023video}. ‘Avg’ denotes the average results for each benchmark. For MSVD-QA, MSRVTT-QA, and ActivityNet-QA benchmarks, only their Acc scores were included in the average calculation. As for ~\cite{maaz2023video}, its average results were used to calculate the final Avg score. }
\label{tab:impact_of_weighted_token_sampler_method}
\end{table}



\usepackage{pgfplots}
\usepackage{ctex}

\pgfplotsset{compat=1.16} 
\begin{document} 
	\begin{tikzpicture}
		\begin{axis}
			[ybar,
			 title={Comparison with different method to sample tokens on MVBench},
			 symbolic x coords={ $S4-V_{10\%_basic}$, $S3-IV_{10\%_basic}$ , $S3-IV_{30\%_basic}$ },
			 legend style={at={(0.55,0.8)}},
			 axis y line=left,
			 axis x line=bottom,
			 nodes near coords,
			 enlarge x limits=0.2, ] 
			\addplot+ coordinates {($S4-V_{10\%_basic}$, 43.52) ($S3-IV_{10\%_basic}$, 1460) ($S3-IV_{30\%_basic}$, 1370); 
			\addplot+ coordinates {($S4-V_{10\%_basic}$, 43.52) ($S3-IV_{10\%_basic}$, 1460) ($S3-IV_{30\%_basic}$, 1370); 
			\legend{basic,diversity}; 
		\end{axis} 
	\end{tikzpicture} 
\end{document}

\begin{table*}[ht]
\center
\begin{small}
\resizebox{0.9\textwidth}{!}
{
\begin{tabular}{c|cccccc|ccccc|c|c}
\toprule
\multirow{2}{*}{\textbf{Method}} & 
\multicolumn{2}{c}{\textbf{MSVD-QA}} & 
\multicolumn{2}{c}{\textbf{MSRVTT-QA}} & 
\multicolumn{2}{c|}{\textbf{ActivityNet-QA}} & 
\multicolumn{5}{c|}{\textbf{Video-based Generative Performance Benchmarking}} &
\multicolumn{1}{c|}{\textbf{Video-Bench}} & 
\textbf{MVBench} \\
& Acc & Score & Acc & Score & Acc & Score & Correctness & Detail & Context & Temporal &  Consistency& Avg&Avg\\
\midrule

S4-V$_{10\%}$  & 69.18 & 3.73 & 55.06 & 3.14 & 49.67 & 3.31 & 2.61 &2.74  & 3.13 & 2.20 &2.29 &50.26 &43.52\\
S4-V$_{30\%}$ & 68.68 &  3.71& 55.13 & 3.16 &48.64  &3.31  & 2.69 & 2.78 & 3.18 & 2.22 & 2.26 & 50.12&44.00\\
S4-V$_{60\%}$  & 68.96 & 3.72 & 55.21 & 3.17 & 48.97 & 3.29 &2.71 &2.79 &3.22  &2.29 & 2.31 
& 50.36&43.73\\
S4-V$_{100\%}$  & 68.57 & 3.70 & 55.20 & 3.17 & 48.85 & 3.31 &2.78 &2.83 &3.23  &2.29 & 2.38 & 50.86&44.47\\
\midrule
S3-IV$_{10\%}$  & 70.25 & 3.77 & 53.36 & 3.13 & 52.22 & 3.39 & 2.69 &2.83  & 3.27 & 2.30 &2.49 &49.70 &44.75\\
S3-IV$_{30\%}$ & 70.39 &  3.78& 55.25 & 3.18 &52.84  &3.41  & 2.64 & 2.80 & 3.20 & 2.35 & 2.49 &48.65 &44.28\\
S3-IV$_{60\%}$  & 69.23 & 3.77 & 54.53 & 3.15 & 52.08 & 3.39 &  2.73    &2.80 &3.25  &2.31 & 2.47 
& 49.89 &44.47\\
S3-IV$_{100\%}$ & 69.55 & 3.78 & 54.50 & 3.17 & 51.54 & 3.40 &2.79 &2.84 &3.29  &2.33 & 2.40 & 48.62&44.30 \\
\midrule
S2-S3-IV$_{10\%-10\%}$  & 68.89 & 3.74 & 51.97 & 3.08 & 51.00 & 3.36 & 2.73 &2.83  & 3.30 & 2.32 &2.46 &50.12 &44.15\\
S2-S3-IV$_{10\%-30\%}$  & 69.51 & 3.75 & 53.77 & 3.15 & 51.75 & 3.41 & 2.76 &2.87  & 3.34 & 2.24 &2.55 &49.90 &44.75\\
S2-S3-IV$_{10\%-60\%}$  & 68.55 & 3.77 & 52.45 & 3.12 & 51.50 & 3.40 & 2.77 &2.85  & 3.32 & 2.28 &2.53 &49.75 &45.78\\
S2-S3-IV$_{10\%-100\%}$ & 69.07 &  3.77& 52.96 & 3.15 &52.45  &3.39  & 2.85 & 2.88 & 3.33 & 2.34 & 2.55 &49.70 &44.80\\
S2-S3-IV$_{100\%-100\%}$  & 69.26 & 3.77 & 54.06 & 3.17 & 52.52 & 3.40 &2.79 &2.85 &3.31  &2.29 & 2.57 &49.97 &44.95\\
\bottomrule
\end{tabular}
}
\end{small}
\caption{Comparison with varying proportions of video training data on Video-QA benchmark,  Video-based Generative Performance benchmark~\cite{maaz2023video}, VideoBench~\cite{ning2023video} and MVBench~\cite{li2023mvbench} benchmark. The resolution of input image and video frame are 448. We sample each frame with 128 tokens.}
\label{tab:impact_of_videodata_amount}
\end{table*}
